Optimizing Library Usage and Browser Experience: Application to the New York Public Library

We tackle the challenge brought to urban library systems by the {holds system} -- which allows users to request books available at other branches to be transferred for local pickup. The holds system increases usage of the entire collection, at the expense of an in-person browser's experience at the source branch. We study the optimization of usage and browser experience, where the library has two levers: where a book should come from when a hold request is placed, and how many book copies at each branch should be available through the holds system versus reserved for browsers. We first show that the problem of maximizing usage can be viewed through the lens of revenue management, for which near-optimal fulfillment policies exist. We then develop a simulation framework that further optimizes for browser experience, through book reservations. We empirically apply our methods to data from the New York Public Library to design implementable policies. We find that though a substantial trade-off exists between these two desiderata, a balanced policy can improve browser experience over the historical policy without significantly sacrificing usage. Because browser usage is more prevalent among branches in low-income areas, this policy further increases system-wide equity: notably, for branches in the 25% lowest-income neighborhoods, it improves both usage and browser experience by about 15%.

==> sections/misc.tex <==
\todo{to delete}

What are the levers of the library?

\begin{enumerate}
    \item Hold fulfillment policy
    \item Amount of inventory reserved for browsers
\end{enumerate}

What are the desiderata of the library?

\begin{enumerate}
    \item Hold user experience: as measured by (1) hold checkouts and (2) fraction of hold requests rejected due to no inventory left for hold fulfillment
    \item Browser experience: as measure by (1) browser checkouts and (2) effective collection quality, which is the summation of desirability of books in stock, does not have to be reserved for browser checkouts (we can think of this as the experience of the people that just read books in the library, they are browsers, but they do not incur checkouts)
\end{enumerate}

Hold user (1) (2) and browser (1) (2) can be directly compared, they are on the same dimension. These are the tradeoffs: we can have two plots here; additionally we know there is at least two points on this plot that serve as the boundary: point A is if all inventory are reserved for browser; point B is if none of the inventory are reserved for browser, and we just maximize checkouts overall.

How do we measure them and get one number?
\begin{enumerate}
    \item hold user (2) can be weighted by the latent demand and the hold usage fraction of each branch
    \item browser (2) can be weighted by the latent demand and (1 - hold usage fraction) of each branch
\end{enumerate}

Link to efficiency - equity tradeoff: we have shown that hold usage correlates with various demographics, prioritizing holds is more efficient for utilization of the books, but we also need to care about browser experience to take care of those neighborhoods.


Plot: map of inflow or outflow


\paragraph{First task:} Model \textbf{Dynamic hold fulfillment + Browser reserve as a parameter} and maximize checkouts 

Tasks:
\begin{itemize}
    \item Writing down the model and policy
    \item Demonstrating the hold-browser tradeoff in this stylized model
\end{itemize}


shortcomings of this modeling: (1) does not tackle reusable resources (this is area of active research) (2) does not provide viable rank-based hold fulfillment policy (3) does not give us more nuanced measures of browser and hold user experience: the effective collection quality and the refusal fraction

\paragraph{Second task:} Use simulation to find the \textbf{Optimal browser reserve} with \textbf{Dynamic hold fulfillment}

Tasks:
\begin{itemize}
    \item Implement this dynamic fulfillment policy within out simulator - DONE
    \item Demonstrate that within the simulator, the dynamic policy achieves almost as good as the theoretical bound under the stylized model (maybe not needed)
    \item Simulation optimization to find the best browser reserves
\end{itemize}

Our modeling is for one book, and the $k_i$ parameter can take any integer from 0 to $c_i$. Maybe have one parameter called the browser reserve fraction $\gamma_i$ for each branch? Such that in the model, we split this branch's inventory into (roughly) $\gamma_i c_i$ and $(1-\gamma_i) c_i$, with $\gamma_i c_i$ reserved for browser usage.

\paragraph{Third task:} Use a \textbf{Static hold fulfillment} to approximate \textbf{Dynamic hold fulfillment}.

How to approximate? (1) Maybe some kind of simple averaging from the outcomes: overall branch $i$ is used for dynamic hold fulfillment

Tasks:
\begin{itemize}
    \item Approximate the fulfillment under the dynamic policy to a rank-based fulfillment
    \item Show (1) comparison to dynamic and (2) comparison to historical
\end{itemize}

% \begin{itemize}
%     \item model: maximize checkouts, such that the inventory does not fall below some threshold
%     \item if we had complete control of the system: dynamic policy
%     \item theory part
% \end{itemize}

% Next:

% \begin{itemize}
%     \item but we do not have complete control of the system
%     \item our real lever is the paging list
% \end{itemize}

% \begin{itemize}
%     \item introduce levers (how to circulate books), the fluid model
%     \item 1/2-approx policy in terms of the total number of checkouts (that is not implementable, or require significant hassle, because it is dynamic)
%     \item introduce the actual decision variables (ranking of branches in the paging list, not changed for long period of time)
%     \item introduce equity objectives (minimize in-flow, out-flow disparities) or constraints
% \end{itemize}

\section{Empirical application}
\begin{itemize}
    \item We have the simulator to simulate the 1/2-approx policy, and compare that with the historical number of checkouts to establish a good upper bound on the total number of checkouts (this 1/2-approx policy is not implementable in practice)
    \item use Bayesian opt to do multi-objective learning, establish the Pareto frontier of optimal policies: the plot we show here would be quite similar to the SLA paper, with the addition of the 1/2-approx policy, which would be even better than this Pareto curve
    \item compare several optimal policies with historical and with 1/2-approx: ideal result is 
    \begin{itemize}
        \item the most efficient comes close to the 1/2-approx, and the most equitable one achieves almost identical net inflow for all branches, which means the class of policy we have is quite flexible
        \item we can achieve good improvement in equity without sacrificing much efficiency, even when compared with the 1/2-approx policy, so the price of equity is not too large
        \item I'm not expecting the implementable policy class to be that flexible yet; although there are some other levers we can use here: e.g., restrict taking books from certain branches during certain periods (lucky days)
    \end{itemize}
    \item show the practical impact of this optimal policy: have a plot for each branch, its gain and loss of total checkouts, and have a plot of the in-flow and out-flow, show that this policy helps flatten the curve
\end{itemize}
